CaLMFlow: Volterra Flow Matching using Causal Language Models

We introduce CaLMFlow (Causal Language Models for Flow Matching), a novel framework that casts flow matching as a Volterra integral equation (VIE), leveraging the power of large language models (LLMs) for continuous data generation. CaLMFlow enables the direct application of LLMs to learn complex flows by formulating flow matching as a sequence modeling task, bridging discrete language modeling and continuous generative modeling. Our method implements tokenization across space and time, thereby solving a VIE over these domains. This approach enables efficient handling of high-dimensional data and outperforms ODE solver-dependent methods like conditional flow matching (CFM). We demonstrate CaLMFlow's effectiveness on synthetic and real-world data, including single-cell perturbation response prediction, showcasing its ability to incorporate textual context and generalize to unseen conditions. Our results highlight LLM-driven flow matching as a promising paradigm in generative modeling, offering improved scalability, flexibility, and context-awareness.

==> figs/cond_single_cell_combined_umaps.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{images/conditional_single_cell/single_cell_conditional_combined_umap_plots.png}
    \caption{Comparison of conditional generation quality across different models for single-cell perturbation data. CaLMFlow exhibits strong overlap between generated data distribution (blue) and the ground-truth distribution (orange), highlighting its superior capability to model data with unseen combinatorial perturbations. In contrast, other models struggle to produce realistic samples. For CaLMFlow, R.I. refers to randomly initialized CLM, and N.L. refers to natural language pretrained CLM.}
    \label{fig:cond_single_cell_combined_umaps}
\end{figure}

==> figs/cond_single_cell_individual_umaps.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{images/conditional_single_cell/single_cell_conditional_individual_umap_plots.png}
    \caption{Comparison of conditional generation quality across different models for single-cell perturbation data. CaLMFlow generates data that accurately reflects the ground truth distribution across all combinatorial labels (cell type, perturbation, and chronicity), demonstrating its superior ability to understand complex conditions while maintaining a realistic overall data distribution. In contrast, methods like CFM-OT, CFM-SB, and scVI generate data where labels are blended, indicating an inability to comprehend conditions. While CFM and scGPT produce well-separated data, it's easily observed that this does not realistically represent the actual distribution when compared to the ground truth.  For CaLMFlow, R.I. refers to randomly initialized CLM, and N.L. refers to natural language pretrained CLM.}
    \label{fig:cond_single_cell_combined_umaps}
\end{figure}

==> figs/mnist_icp.tex <==
\begin{figure}[t]\centering

    \includegraphics[width=0.24\textwidth]{images/conditional_mnist/mnist_inception_plot.png}
    \caption{Inception scores for MNIST} 
    \label{fig:conditional_mnist}
\end{figure}

==> tabs/high_dim_toy_dataset.tex <==
\begin{table}[t]
\centering
\small
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{lcccccc}
    \toprule
    
    % & \multicolumn{6}{c}{\textbf{Dimension}} \\
    Data Dimension $\rightarrow$ & \multicolumn{2}{c}{10} & \multicolumn{2}{c}{100} & \multicolumn{2}{c}{1000} \\
    \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
    
    Method $\downarrow$ Metric  $\rightarrow$ & 2-Wass ($\downarrow$) & MMD ($\downarrow$) & 2-Wass ($\downarrow$)& MMD ($\downarrow$) & 2-Wass ($\downarrow$) & MMD ($\downarrow$) \\
    
    \midrule
    \multicolumn{1}{c}{} & \multicolumn{6}{c}{Gaussian $\rightarrow$ 2 Gaussians} \\
    \cmidrule(lr){2-7}
    CFM & $1.407 \text{ \scriptsize{$\pm$0.379}}$ & \textbf{0.025}$ \text{ \scriptsize{$\pm$0.001}}$ & $5.483 \text{ \scriptsize{$\pm$0.569}}$ & $0.324 \text{ \scriptsize{$\pm$0.001}}$ & $25.064 \text{ \scriptsize{$\pm$1.291}}$ & $0.488 \text{ \scriptsize{$\pm$0.001}}$ \\
    CFM-OT & \textbf{1.096}$ \text{ \scriptsize{$\pm$0.317}}$ & $0.028 \text{ \scriptsize{$\pm$0.001}}$ & $5.494 \text{ \scriptsize{$\pm$0.517}}$ & 0.322$ \text{ \scriptsize{$\pm$0.001}}$ & $25.131 \text{ \scriptsize{$\pm$1.209}}$ & $0.490 \text{ \scriptsize{$\pm$0.001}}$ \\
    CFM-SB & \textbf{1.057}$ \text{ \scriptsize{$\pm$0.339}}$ & $0.029 \text{ \scriptsize{$\pm$0.002}}$ & $5.504 \text{ \scriptsize{$\pm$0.446}}$ & $0.336 \text{ \scriptsize{$\pm$0.001}}$ & 25.053$ \text{ \scriptsize{$\pm$1.558}}$ & $0.493 \text{ \scriptsize{$\pm$0.001}}$ \\
    % CaLMFlow ($\tau=1$) & \textbf{1.050}$ \text{ \scriptsize{$\pm$0.408}}$ & $0.114 \text{ \scriptsize{$\pm$0.002}}$ & \textbf{3.406}$ \text{ \scriptsize{$\pm$1.081}}$ & $0.291 \text{ \scriptsize{$\pm$0.003}}$ & $15.828 \text{ \scriptsize{$\pm$4.203}}$ & $0.317 \text{ \scriptsize{$\pm$0.001}}$ \\
    % CaLMFlow ($\tau=2$) & $1.133 \text{ \scriptsize{$\pm$0.290}}$ & $0.067 \text{ \scriptsize{$\pm$0.003}}$ & \textbf{3.137}$ \text{ \scriptsize{$\pm$1.028}}$ & $0.211 \text{ \scriptsize{$\pm$0.003}}$ & $15.694 \text{ \scriptsize{$\pm$4.086}}$ & \textbf{0.317}$ \text{ \scriptsize{$\pm$0.001}}$ \\
    % CaLMFlow ($\tau=5$) & $1.317 \text{ \scriptsize{$\pm$0.291}}$ & $0.060 \text{ \scriptsize{$\pm$0.003}}$ & $3.372 \text{ \scriptsize{$\pm$0.907}}$ & $0.099 \text{ \scriptsize{$\pm$0.003}}$ & $14.078 \text{ \scriptsize{$\pm$3.926}}$ & \textbf{0.303}$ \text{ \scriptsize{$\pm$0.002}}$ \\
    % CaLMFlow ($\tau=10$)& $1.931 \text{ \scriptsize{$\pm$0.195}}$ & $0.109 \text{ \scriptsize{$\pm$0.003}}$ & $3.856 \text{ \scriptsize{$\pm$0.859}}$ & $0.117 \text{ \scriptsize{$\pm$0.003}}$ & \textbf{11.027}$ \text{ \scriptsize{$\pm$3.853}}$ & \textbf{0.261}$ \text{ \scriptsize{$\pm$0.003}}$ \\
    \midrule

    CaLMFlow        & \textbf{1.050}$ \text{ \scriptsize{$\pm$0.408}}$ & $0.060 \text{ \scriptsize{$\pm$0.002}}$ & \textbf{3.137}$ \text{ \scriptsize{$\pm$1.028}}$ & $\textbf{0.211} \text{ \scriptsize{$\pm$0.003}}$ & \textbf{11.027}$ \text{ \scriptsize{$\pm$3.853}}$ & \textbf{0.261}$ \text{ \scriptsize{$\pm$0.003}}$ \\
    
    \midrule
    \multicolumn{1}{c}{} & \multicolumn{6}{c}{Gaussian $\rightarrow$ 8 Gaussians} \\
    \cmidrule(lr){2-7}
    CFM & $0.621 \text{ \scriptsize{$\pm$0.070}}$ & 0.018$ \text{ \scriptsize{$\pm$0.001}}$ & $4.846 \text{ \scriptsize{$\pm$0.054}}$ & $0.224 \text{ \scriptsize{$\pm$0.005}}$ & $23.294 \text{ \scriptsize{$\pm$0.166}}$ & $0.402 \text{ \scriptsize{$\pm$0.004}}$ \\
    CFM-OT & \textbf{0.439}$ \text{ \scriptsize{$\pm$0.023}}$ & \textbf{0.017}$ \text{ \scriptsize{$\pm$0.001}}$ & 4.795$ \text{ \scriptsize{$\pm$0.031}}$ & $0.227 \text{ \scriptsize{$\pm$0.004}}$ & 23.116$ \text{ \scriptsize{$\pm$0.118}}$ & $0.407 \text{ \scriptsize{$\pm$0.003}}$ \\
    CFM-SB & $0.550 \text{ \scriptsize{$\pm$0.061}}$ & \textbf{0.016}$ \text{ \scriptsize{$\pm$0.001}}$ & $4.914 \text{ \scriptsize{$\pm$0.038}}$ & $0.236 \text{ \scriptsize{$\pm$0.005}}$ & $23.211 \text{ \scriptsize{$\pm$0.078}}$ & $0.412 \text{ \scriptsize{$\pm$0.003}}$ \\
    % CaLMFlow ($\tau=1$) & $1.060 \text{ \scriptsize{$\pm$0.068}}$ & $0.027 \text{ \scriptsize{$\pm$0.001}}$ & $3.207 \text{ \scriptsize{$\pm$0.161}}$ & $0.064 \text{ \scriptsize{$\pm$0.002}}$ & $13.708 \text{ \scriptsize{$\pm$0.290}}$ & $0.099 \text{ \scriptsize{$\pm$0.001}}$ \\
    % CaLMFlow ($\tau=2$) & $0.926 \text{ \scriptsize{$\pm$0.067}}$ & $0.026 \text{ \scriptsize{$\pm$0.002}}$ & $2.884 \text{ \scriptsize{$\pm$0.195}}$ & $0.043 \text{ \scriptsize{$\pm$0.002}}$ & $12.836 \text{ \scriptsize{$\pm$0.302}}$ & $0.097 \text{ \scriptsize{$\pm$0.001}}$ \\
    % CaLMFlow ($\tau=5$) & $1.320 \text{ \scriptsize{$\pm$0.032}}$ & $0.075 \text{ \scriptsize{$\pm$0.003}}$ & \textbf{2.317}$ \text{ \scriptsize{$\pm$0.226}}$ & \textbf{0.014}$ \text{ \scriptsize{$\pm$0.001}}$ & $10.646 \text{ \scriptsize{$\pm$0.306}}$ & \textbf{0.088}$ \text{ \scriptsize{$\pm$0.001}}$ \\
    % CaLMFlow ($\tau=10$) & $2.324 \text{ \scriptsize{$\pm$0.048}}$ & $0.120 \text{ \scriptsize{$\pm$0.002}}$ & $2.484 \text{ \scriptsize{$\pm$0.263}}$ & $0.018 \text{ \scriptsize{$\pm$0.002}}$ & \textbf{8.272}$ \text{ \scriptsize{$\pm$0.272}}$ & \textbf{0.073}$ \text{ \scriptsize{$\pm$0.001}}$ \\
    \midrule

    CaLMFlow  & $0.926 \text{ \scriptsize{$\pm$0.067}}$ & $0.026 \text{ \scriptsize{$\pm$0.002}}$ & \textbf{2.317}$ \text{ \scriptsize{$\pm$0.226}}$ & \textbf{0.014}$ \text{ \scriptsize{$\pm$0.001}}$ & \textbf{8.272}$ \text{ \scriptsize{$\pm$0.272}}$ & \textbf{0.073}$ \text{ \scriptsize{$\pm$0.001}}$ \\
    
    \midrule
    \multicolumn{1}{c}{} & \multicolumn{6}{c}{Gaussian $\rightarrow$ 2 Moons} \\
    \cmidrule(lr){2-7}
    CFM & 0.570$ \text{ \scriptsize{$\pm$0.099}}$ & \textbf{0.011}$ \text{ \scriptsize{$\pm$0.001}}$ & $5.061 \text{ \scriptsize{$\pm$0.103}}$ & $0.194 \text{ \scriptsize{$\pm$0.004}}$ & $23.428 \text{ \scriptsize{$\pm$0.187}}$ & $0.363 \text{ \scriptsize{$\pm$0.002}}$ \\
    CFM-OT & $0.576 \text{ \scriptsize{$\pm$0.096}}$ & \textbf{0.011}$ \text{ \scriptsize{$\pm$0.001}}$ & $5.013 \text{ \scriptsize{$\pm$0.058}}$ & $0.195 \text{ \scriptsize{$\pm$0.004}}$ & 23.339$ \text{ \scriptsize{$\pm$0.133}}$ & $0.363 \text{ \scriptsize{$\pm$0.003}}$ \\
    CFM-SB & \textbf{0.555}$ \text{ \scriptsize{$\pm$0.051}}$ & $0.013 \text{ \scriptsize{$\pm$0.001}}$ & $5.294 \text{ \scriptsize{$\pm$0.042}}$ & $0.218 \text{ \scriptsize{$\pm$0.004}}$ & $23.805 \text{ \scriptsize{$\pm$0.132}}$ & $0.373 \text{ \scriptsize{$\pm$0.004}}$ \\
    % CaLMFlow ($\tau=1$) & $0.967 \text{ \scriptsize{$\pm$0.083}}$ & $0.014 \text{ \scriptsize{$\pm$0.001}}$ & $4.248 \text{ \scriptsize{$\pm$0.128}}$ & $0.032 \text{ \scriptsize{$\pm$0.001}}$ & $15.667 \text{ \scriptsize{$\pm$0.220}}$ & $0.049 \text{ \scriptsize{$\pm$0.001}}$ \\
    % CaLMFlow ($\tau=2$) & $0.822 \text{ \scriptsize{$\pm$0.092}}$ & $0.013 \text{ \scriptsize{$\pm$0.001}}$ & $3.960 \text{ \scriptsize{$\pm$0.138}}$ & $0.025 \text{ \scriptsize{$\pm$0.001}}$ & $15.220 \text{ \scriptsize{$\pm$0.206}}$ & $0.048 \text{ \scriptsize{$\pm$0.001}}$ \\
    % CaLMFlow ($\tau=5$) & $1.184 \text{ \scriptsize{$\pm$0.092}}$ & $0.039 \text{ \scriptsize{$\pm$0.001}}$ & \textbf{3.283}$ \text{ \scriptsize{$\pm$0.175}}$ & \textbf{0.014}$ \text{ \scriptsize{$\pm$0.001}}$ & $14.493 \text{ \scriptsize{$\pm$0.255}}$ & \textbf{0.046}$ \text{ \scriptsize{$\pm$0.001}}$ \\
    % CaLMFlow ($\tau=10$) & $1.996 \text{ \scriptsize{$\pm$0.053}}$ & $0.077 \text{ \scriptsize{$\pm$0.002}}$ & \textbf{2.944}$ \text{ \scriptsize{$\pm$0.195}}$ & $0.018 \text{ \scriptsize{$\pm$0.002}}$ & \textbf{13.423}$ \text{ \scriptsize{$\pm$0.258}}$ & \textbf{0.039}$ \text{ \scriptsize{$\pm$0.001}}$ \\
    \midrule
    
    CaLMFlow  & $0.822 \text{ \scriptsize{$\pm$0.092}}$ & $0.013 \text{ \scriptsize{$\pm$0.001}}$ & \textbf{2.944}$ \text{ \scriptsize{$\pm$0.195}}$ & $\textbf{0.018} \text{ \scriptsize{$\pm$0.002}}$ & \textbf{13.423}$ \text{ \scriptsize{$\pm$0.258}}$ & \textbf{0.039}$ \text{ \scriptsize{$\pm$0.001}}$ \\

    \bottomrule
\end{tabular}
\end{adjustbox}
\caption{
    Comparison of different CFM variants and CaLMFlow across distribution pairs ($\mu \pm \sigma$ over five seeds) in terms of fit (2-Wasserstein) and MMD. Best results in bold.
}
\label{tab:high_dim_toy_data}
\end{table}

==> tabs/multipoint_toy_dataset_wrap.tex <==
\begin{wraptable}[20]{r}{0.5\textwidth}
\centering
\small
\begin{adjustbox}{width=0.5\textwidth}
\begin{tabular}{lccc}
    \toprule
          
    Method $\downarrow$ Metric  $\rightarrow$ & 2-Wass ($\downarrow$) & MMD ($\downarrow$) \\
    
    % \midrule
    % \multicolumn{1}{c}{} & \multicolumn{2}{c}{2 Moons $\rightarrow$ 8 Gaussians in 2 Dimensions} \\
    % \cmidrule(lr){2-3}
    % CFM & {1.0948 $\pm$ 0.0631} & {0.0025 $\pm$ 0.0002} \\
    % CaLMFlow (1 point) & {1.3756 $\pm$ 0.0668} & {0.0057 $\pm$ 0.0002} \\
    % % CaLMFlow (4 points) & {1.0477 $\pm$ 0.0771} & {0.0041 $\pm$ 0.0003} \\
    % CaLMFlow (10 points) & \textbf{0.8753 $\pm$ 0.1243} & \textbf{0.0020 $\pm$ 0.0003} \\
    
    \midrule
    \multicolumn{1}{c}{} & \multicolumn{2}{c}{2 Gaussians $\rightarrow$ 3 Gaussians in 100 Dimensions} \\
    \cmidrule(lr){2-3}
    CFM & {6.4344 $\pm$ 0.2738} & {0.0293 $\pm$ 0.0008} \\
    CaLMFlow (1 traj.) & {4.0898 $\pm$ 0.1842} & {0.02021 $\pm$ 0.0016} \\
    CaLMFlow (8 traj.) & \textbf{2.8363 $\pm$ 0.3868} & \textbf{0.0149 $\pm$ 0.0016} \\
        
    \midrule
    \multicolumn{1}{c}{} & \multicolumn{2}{c}{2 Gaussians $\rightarrow$ 4 Gaussians in 100 Dimensions} \\
    \cmidrule(lr){2-3}
    CFM & {6.3400 $\pm$ 0.3185} & {0.0206 $\pm$ 0.0003} \\
    CaLMFlow (1 traj.) & {5.6608 $\pm$ 0.3272} & {0.0148 $\pm$ 0.0007} \\
    CaLMFlow (8 traj.) & \textbf{3.6119 $\pm$ 0.3213} & \textbf{0.0058 $\pm$ 0.0005} \\
    
    \bottomrule
    
\end{tabular}
\end{adjustbox}
\caption{
    % Comparison of CFM, CaLMFlow and CaLMFlow-multi-trajectories across distributions pairs ($\mu \pm \sigma$ over 5 runs) in terms of fit (2-Wasserstein) and MMD. Best results in bold.
     Comparisons of CFM, CaLMFlow, and CaLMFlow with multiple trajectories on different distribution pairs in 100 dimensions. We report 2-Wasserstein distance (2-Wass) and Maximum Mean Discrepancy (MMD), averaged over 5 runs. Best results are highlighted in bold. The table shows that CaLMFlow, especially when utilizing multiple trajectories, significantly outperforms CFM in terms of both fit and distribution accuracy. This demonstrates the advantage of leveraging multi-trajectory modeling in CaLMFlow.
}
\label{tab:multi_point}
\end{wraptable}
